FSM Error Messages

Computer Science students, in general, find Automata Theory difficult and mostly unrelated to their area of study. To mitigate these perceptions, FSM, a library to program state machines and grammars, was developed to bring programming to the Automata Theory classroom. The results of the library's maiden voyage at Seton Hall University had a positive impact on students, but the students found the library difficult to use due to the error messages generated. These messages were generated by the host language meaning that students needed to be familiar with the library's implementation to make sense of them. This article presents the design of and results obtained from using an error-messaging system tailor-made for FSM. The effectiveness of the library was measured by both a control group study and a survey. The results strongly suggest that the error-messaging system has had a positive impact on students' attitude towards automata theory, towards programming in FSM, and towards FSM error messages. The consequence has been a marked improvement on students' ability to implement algorithms developed as part of constructive proofs by making the debugging of FSM programs easier.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{P. Achten, H. Miller (Eds.): \\
Trends in Functional Programming in Education 2018 (TFPIE'18)\\
EPTCS 295, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.295.1}{10.4204/EPTCS.295.1}}
\pdfoutput=1

